Production, Quality Assurance and Quality Control of the SiPM Tiles for the DarkSide-20k Time Projection Chamber

The DarkSide-20k dark matter direct detection experiment will employ a 21 m^2 silicon photomultiplier (SiPM) array, instrumenting a dual-phase 50 tonnes liquid argon Time Projection Chamber (TPC). SiPMs are arranged into modular photosensors called Tiles, each integrating 24 SiPMs onto a printed circuit board (PCB) that provides signal amplification, power distribution, and a single-ended output for simplified readout. 16 Tiles are further grouped into Photo-Detector Units (PDUs). This paper details the production of the Tiles and the quality assurance and quality control (QA-QC) protocol established to ensure their performance and uniformity. The production and QA-QC of the Tiles are carried out at Nuova Officina Assergi (NOA), an ISO-6 clean room facility at LNGS. This process includes wafer-level cryogenic characterisation, precision flip-chip bonding, wire bonding, and extensive electrical and optical validation of each Tile. The overall production yield exceeds 83.5%, matching the requirements of the DarkSide-20k production plan. These results validate the robustness of the Tile design and its suitability for operation in a cryogenic environment.

==> authors_June2025.tex <==
%\renewcommand{\thanksref}[1]{$^{\ref{#1}}$}
\newcommand{\notds}{\nolinebreak\footnotemark\nolinebreak}
\renewcommand{\thefootnote}{$*$}
{
\onecolumn
\textbf{The DarkSide-20k Collaboration}


F.~Acerbi\thanksref{l_TNFBK}\nolinebreak,
P.~Adhikari\thanksref{l_Carleton}\nolinebreak,
P.~Agnes\thanksref{l_AQGSSI}\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
I.~Ahmad\thanksref{l_AstroCeNT}\nolinebreak,
S.~Albergo\thanksref{l_CTUNI}\textsuperscript{,}\thanksref{l_CTINFN}\nolinebreak,
I.~F.~Albuquerque\thanksref{l_USP}\nolinebreak,
T.~Alexander\thanksref{l_PNNL}\nolinebreak,
A.~K.~Alton\thanksref{l_Augustana}\nolinebreak,
P.~Amaudruz\thanksref{l_TRIUMF}\nolinebreak,
M.~Angiolilli\thanksref{l_AQGSSI}\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
E.~Aprile\thanksref{l_Columbia}\nolinebreak,
M.~Atzori Corona\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{l_CAUniPHY}\nolinebreak, %GRACE PERIOD END 02-2026
D.~J.~Auty\thanksref{l_Alberta}\nolinebreak,
M.~Ave\thanksref{l_AQGSSI}\textsuperscript{,}\thanksref{l_USP}\nolinebreak,
I.~C.~Avetisov\thanksref{l_MendeleevUniverisity}\nolinebreak,
O.~Azzolini\thanksref{l_LNLINFN}\nolinebreak,
H.~O.~Back\thanksref{l_PNNL}\textsuperscript{,}\thanksref{l_SNOLAB}\nolinebreak,
Z.~Balmforth\thanksref{l_UniHAM}\nolinebreak,
A.~Barrado Olmedo\thanksref{l_CIEMAT}\nolinebreak,
P.~Barrillon\thanksref{l_CPPM}\nolinebreak,
G.~Batignani\thanksref{l_PIUniPHY}\textsuperscript{,}\thanksref{l_PIINFN}\nolinebreak,
P.~Bhowmick\thanksref{l_Oxford}\nolinebreak,
M.~Bloem\thanksref{l_STFCppd}\nolinebreak,
S.~Blua\thanksref{l_TOINFN}\textsuperscript{,}\thanksref{l_TOPoli}\nolinebreak,
V.~Bocci\thanksref{l_RMUnoINFN}\nolinebreak,
W.~Bonivento\thanksref{l_CAINFN}\nolinebreak,
B.~Bottino\thanksref{l_GEUni}\textsuperscript{,}\thanksref{l_GEINFN}\nolinebreak,
M.~G.~Boulay\thanksref{l_Carleton}\nolinebreak,
T.~Braun\thanksref{l_Oxford}\nolinebreak,
A.~Buchowicz\thanksref{l_WUT}\nolinebreak,
S.~Bussino\thanksref{l_RMTreINFN}\textsuperscript{,}\thanksref{l_RMTreUni}\nolinebreak,
J.~Busto\thanksref{l_CPPM}\nolinebreak,
M.~Cadeddu\thanksref{l_CAINFN}\nolinebreak,
M.~Cadoni\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{l_CAUniPHY}\nolinebreak,
R.~Calabrese\thanksref{l_NAUniPHY}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak,
V.~Camillo\thanksref{l_VTech}\nolinebreak,
A.~Caminata\thanksref{l_GEINFN}\nolinebreak,
N.~Canci\thanksref{l_NAINFN}\nolinebreak,
M.~Caravati\thanksref{l_AQGSSI}\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
M.~Cárdenas-Montes\thanksref{l_CIEMAT}\nolinebreak,
N.~Cargioli\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{l_CAUniPHY}\nolinebreak,
M.~Carlini\thanksref{l_AQLNGS}\nolinebreak,
A.~Castellani\thanksref{l_MIPoliICA}\textsuperscript{,}\thanksref{l_MIINFN}\nolinebreak,
%P.~Castello\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{\CAUniEEE}
P.~Cavalcante\thanksref{l_AQLNGS}\nolinebreak,
S.~Cebrian\thanksref{l_Zaragoza}\nolinebreak,
S.~Chashin\thanksref{l_MSU}\nolinebreak,
A.~Chepurnov\thanksref{l_MSU}\nolinebreak,
S.~Choudhary\thanksref{l_AstroCeNT}\nolinebreak,
L.~Cifarelli\thanksref{l_BOUniPHY}\textsuperscript{,}\thanksref{l_BOINFN}\nolinebreak,
B.~Cleveland\thanksref{l_Laurentian}\textsuperscript{,}\thanksref{l_SNOLAB}  %--> END of grace period 4/11/2025
Y.~Coadou\thanksref{l_CPPM}\nolinebreak,
V.~Cocco\thanksref{l_CAINFN}\nolinebreak,
D.~Colaiuda\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_UnivAQ}\nolinebreak,
E.~Conde Vilda\thanksref{l_CIEMAT}\nolinebreak,
L.~Consiglio\thanksref{l_AQLNGS}\nolinebreak,
B.~S.~Costa\thanksref{l_USP}\nolinebreak,
M.~Czubak\thanksref{l_Krakow}\nolinebreak,
M.~D'Aniello\thanksref{l_NAUniDIST}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak,
S.~D'Auria\thanksref{l_MIUni}\textsuperscript{,}\thanksref{l_MIINFN}\nolinebreak,
M.~D.~Da Rocha Rolo\thanksref{l_TOINFN}\nolinebreak,
A.~Dainty\thanksref{l_STFCInterconnect} \nolinebreak,
G.~Darbo\thanksref{l_GEINFN}\nolinebreak,
S.~Davini\thanksref{l_GEINFN}\nolinebreak,
R.~de Asmundis\thanksref{l_NAINFN}\nolinebreak,
S.~De Cecco\thanksref{l_RMUnoUni}\textsuperscript{,}\thanksref{l_RMUnoINFN}\nolinebreak,
G.~Dellacasa\thanksref{l_TOINFN}\nolinebreak,
A.~V.~Derbin\thanksref{l_Petersburg}\nolinebreak,
A.~Devoto\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{l_CAUniPHY}\nolinebreak,
%F.~Di Capua\thanksref{l_NAUniPHY}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak, %GRACE PERIOD 1 Jun 2025
L.~Di Noto\thanksref{l_GEUni}\textsuperscript{,}\thanksref{l_GEINFN}\nolinebreak,
P.~Di Stefano\thanksref{l_Queens}\nolinebreak,
L.~K.~Dias\thanksref{l_USP}\nolinebreak,
D.~Díaz Mairena\thanksref{l_CIEMAT} \nolinebreak,
C.~Dionisi\thanksref{l_RMUnoUni}\textsuperscript{,}\thanksref{l_RMUnoINFN}\nolinebreak,
G.~Dolganov\thanksref{l_Kurchatov}\textsuperscript{,}\thanksref{l_MEPhI}\nolinebreak,
F.~Dordei\thanksref{l_CAINFN}\nolinebreak,
V.~Dronik\thanksref{l_Belgorod}\nolinebreak,  % END GRACE PERIOD 01/11/2025
F.~Dylon\thanksref{l_UCDavis}\nolinebreak,
A.~Elersich\thanksref{l_UCDavis}\nolinebreak,
E.~Ellingwood\thanksref{l_Queens}\nolinebreak,  % END GRACE PERIOD 01/09/2025
T.~Erjavec\thanksref{l_UCDavis}\nolinebreak,
N.~Fearon\thanksref{l_Oxford}\nolinebreak,
M.~Fernandez Diaz\thanksref{l_CIEMAT}\nolinebreak,
A.~Ficorella\thanksref{l_TNFBK}\nolinebreak,
G.~Fiorillo\thanksref{l_NAUniPHY}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak,
D.~Fleming\thanksref{l_UCDavis}\nolinebreak,
P.~Franchini\thanksref{l_Oxford}\nolinebreak,
D.~Franco\thanksref{l_APC}\nolinebreak,
H.~Frandini Gatti\thanksref{l_Liverpool}\nolinebreak,
E.~Frolov\thanksref{l_BINP}\nolinebreak, % END OF GRACE PERIOD Nov. 1, 2025
F.~Gabriele\thanksref{l_CAINFN}\nolinebreak,
D.~Gahan\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{l_CAUniPHY}\nolinebreak,
C.~Galbiati\thanksref{l_Princeton}\nolinebreak,
G.~Galiński\thanksref{l_WUT}\nolinebreak,
G.~Gallina\thanksref{l_Princeton}\nolinebreak,
%G.~Gallus\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{\CAUniEEE}
M.~Garbini\thanksref{l_BOCentroFermi}\textsuperscript{,}\thanksref{l_BOINFN}\nolinebreak,
P.~Garcia Abia\thanksref{l_CIEMAT}\nolinebreak,
A.~Gawdzik\thanksref{l_Manchester}\nolinebreak,
A.~Gendotti\thanksref{l_ETHZ}\nolinebreak,G.~K.~Giovanetti\thanksref{l_WilliamsCollege}\nolinebreak,
V.~Goicoechea Casanueva\thanksref{l_Hawaii}\nolinebreak,
A.~Gola\thanksref{l_TNFBK}\nolinebreak,
L.~Grandi\thanksref{l_Chicago}\nolinebreak,
G.~Grauso\thanksref{l_NAINFN}\nolinebreak,
G.~Grilli di Cortona\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_RMUnoINFN}\nolinebreak,
A.~Grobov\thanksref{l_Kurchatov}\nolinebreak,
M.~Gromov\thanksref{l_MSU}\nolinebreak,
M.~Gulino\thanksref{l_CTLNS}\textsuperscript{,}\thanksref{l_ENUniCEE}
B.~R.~Hackett\thanksref{l_PNNL}\nolinebreak,
A.~L.~Hallin\thanksref{l_Alberta}\nolinebreak,
A.~Hamer\thanksref{l_UniversityofEdinburgh}\nolinebreak, % END OF GRACE PERIOD 30/09/2025
M.~Haranczyk\thanksref{l_Krakow}\nolinebreak,
B.~Harrop\thanksref{l_Princeton}\nolinebreak,
T.~Hessel\thanksref{l_APC}\nolinebreak,
C.~Hidalgo\thanksref{l_AQGSSI}\nolinebreak,
J.~Hollingham\thanksref{l_STFCInterconnect}\nolinebreak, % TO BE CHECKED!!!!!!
S.~Horikawa\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_UnivAQ}
J.~Hu\thanksref{l_Alberta}\nolinebreak, 
F.~Hubaut\thanksref{l_CPPM}\nolinebreak, 
D.~Huff\thanksref{l_Houston}\nolinebreak, 
T.~Hugues\thanksref{l_Queens}\nolinebreak,   %\thanksref{l_AstroCeNT} Ended 12/2023 thanksref Queens start 1/2024 --> added to DB 
E.~V.~Hungerford\thanksref{l_Houston}\nolinebreak,
A.~Ianni\thanksref{l_Princeton}\nolinebreak,
A.~Ianni\thanksref{l_AQLNGS}\nolinebreak,
V.~Ippolito\thanksref{l_RMUnoINFN}\nolinebreak,
A.~Jamil\thanksref{l_Princeton}\nolinebreak,
C.~Jillings\thanksref{l_Laurentian}\textsuperscript{,}\thanksref{l_SNOLAB}\nolinebreak,
R.~Keloth\thanksref{l_VTech}\nolinebreak,
N.~Kemmerich\thanksref{l_USP}\nolinebreak,
A.~Kemp\thanksref{l_STFCppd} %\thanksref{l_Queens}\nolinebreak,
M.~Kimura\thanksref{l_AstroCeNT}\nolinebreak, %End of grace period Nov. 21, 2025
A.~Klenin\thanksref{l_Belgorod}\nolinebreak, 
K.~Kondo\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_UnivAQ}\nolinebreak,
G.~Korga\thanksref{l_RHUL}\nolinebreak,
L.~Kotsiopoulou\thanksref{l_UniversityofEdinburgh}\nolinebreak,
S.~Koulosousas\thanksref{l_RHUL}\nolinebreak,
A.~Kubankin\thanksref{l_Belgorod}\nolinebreak,
P.~Kunzé\thanksref{l_AQGSSI}\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
M.~Kuss\thanksref{l_PIINFN}\nolinebreak,
M.~Kuźniak\thanksref{l_AstroCeNT}\nolinebreak,
M.~Kuzwa\thanksref{l_AstroCeNT}\nolinebreak,
M.~La Commara\thanksref{l_NAUniPHARM}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak,
M.~Lai\thanksref{l_UCRiverside}\nolinebreak,
E.~Le Guirriec\thanksref{l_CPPM}\nolinebreak,
E.~Leason\thanksref{l_Oxford}\nolinebreak,
A.~Leoni\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_UnivAQ}\nolinebreak,
L.~Lidey\thanksref{l_PNNL}\nolinebreak,
J.~Lipp\thanksref{l_STFCInterconnect}\nolinebreak,
M.~Lissia\thanksref{l_CAINFN}\nolinebreak,
L.~Luzzi\thanksref{l_UCDavis}\nolinebreak,
O.~Lychagina\thanksref{l_JINR}\nolinebreak,
O.~Macfadyen\thanksref{l_RHUL}\nolinebreak,
I.~Machts\thanksref{l_APC}\nolinebreak,
I.~N.~Machulin\thanksref{l_Kurchatov}\textsuperscript{,}\thanksref{l_MEPhI}\nolinebreak,
S.~Manecki\thanksref{l_Laurentian}\textsuperscript{,}\thanksref{l_SNOLAB}\nolinebreak,
I.~Manthos\thanksref{l_UniHAM}\nolinebreak,
L.~Mapelli\thanksref{l_Princeton} \nolinebreak,
A.~Marasciulli\thanksref{l_AQLNGS} %\thanksref{l_PIINFN}\nolinebreak,
S.~M.~Mari\thanksref{l_RMTreINFN}\textsuperscript{,}\thanksref{l_RMTreUni}\nolinebreak,
C.~Mariani\thanksref{l_VTech}\nolinebreak,
J.~Maricic\thanksref{l_Hawaii}\nolinebreak,
M.~Martinez\thanksref{l_Zaragoza}\nolinebreak,
C.~J.~Martoff\thanksref{l_Temple}\textsuperscript{,}\thanksref{l_PNNL}\nolinebreak,
G.~Matteucci\thanksref{l_NAUniPHY}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak,
K.~Mavrokoridis\thanksref{l_Liverpool}\nolinebreak,
A.~B.~McDonald\thanksref{l_Queens}\nolinebreak,
S.~Merzi\thanksref{l_TNFBK}\nolinebreak,
A.~Messina\thanksref{l_RMUnoUni}\textsuperscript{,}\thanksref{l_RMUnoINFN}\nolinebreak,
R.~Milincic\thanksref{l_Hawaii}\nolinebreak,
S.~Minutoli\thanksref{l_GEINFN}\nolinebreak,
A.~Mitra\thanksref{l_Warwick}\nolinebreak,
J.~Monroe\thanksref{l_Oxford}\nolinebreak,
E.~Moretti\thanksref{l_TNFBK}\nolinebreak,
M.~Morrocchi\thanksref{l_PIUniPHY}\textsuperscript{,}\thanksref{l_PIINFN}\nolinebreak,
A.~Morsy\thanksref{l_UMass}\nolinebreak,
T.~Mroz\thanksref{l_Krakow} \nolinebreak,  %end grace period 2025-08-31
V.~N.~Muratova\thanksref{l_Petersburg}\nolinebreak,
M.~Murra\thanksref{l_Columbia}\nolinebreak,
%C.~Muscas\thanksref{\CAINFN\thanksref{\CAUniEEE}\nolinebreak,
P.~Musico\thanksref{l_GEINFN}\nolinebreak,
R.~Nania\thanksref{l_BOINFN}\nolinebreak,
M.~Nessi\thanksref{l_INFN}\nolinebreak,
G.~Nieradka\thanksref{l_AstroCeNT}\nolinebreak,
K.~Nikolopoulos\thanksref{l_UniHAM} \nolinebreak,%\thanksref{\Birmingham}
E.~Nikoloudaki\thanksref{l_APC}\nolinebreak,
I.~Nikulin\thanksref{l_Belgorod}\nolinebreak,
J.~Nowak\thanksref{l_Lancaster}\nolinebreak,
K.~Olchanski\thanksref{l_TRIUMF}
A.~Oleinik\thanksref{l_Belgorod}\nolinebreak,
V.~Oleynikov\thanksref{l_BINP}\nolinebreak,
P.~Organtini\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_Princeton}\nolinebreak,
A.~Ortiz~de~Solórzano\thanksref{l_Zaragoza}\nolinebreak,
A.~Padmanabhan\thanksref{l_Queens} \nolinebreak,
M.~Pallavicini\thanksref{l_GEUni}\textsuperscript{,}\thanksref{l_GEINFN}\nolinebreak,
L.~Pandola\thanksref{l_CTLNS}\nolinebreak,
E.~Pantic\thanksref{l_UCDavis}\nolinebreak,
E.~Paoloni\thanksref{l_PIUniPHY}\textsuperscript{,}\thanksref{l_PIINFN}\nolinebreak,
D.~Papi\thanksref{l_Alberta}\nolinebreak,
B.~Park\thanksref{l_Alberta}\nolinebreak,
G.~Pastuszak\thanksref{l_WUT}\nolinebreak,
G.~Paternoster\thanksref{l_TNFBK}\nolinebreak,
A.~Peck\thanksref{l_UCRiverside}\nolinebreak,
%P.~A.~Pegoraro\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{\CAUniEEE}
K.~Pelczar\thanksref{l_Krakow}\nolinebreak,
R.~Perez\thanksref{l_USP}\nolinebreak,
V.~Pesudo\thanksref{l_CIEMAT}\nolinebreak,
S.~Piacentini\thanksref{l_AQGSSI}\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
N.~Pino\thanksref{l_CTLNS}\nolinebreak,%\thanksref{\CTUNI\thanksref{l_CTINFN}
G.~Plante\thanksref{l_Columbia}\nolinebreak,
A.~Pocar\thanksref{l_UMass}\nolinebreak,
S.~Pordes\thanksref{l_VTech}\nolinebreak,
P.~Pralavorio\thanksref{l_CPPM}\nolinebreak,
E.~Preosti\thanksref{l_Princeton}\nolinebreak,
D.~Price\thanksref{l_Manchester}\nolinebreak,
M.~Pronesti\thanksref{l_CPPM}\nolinebreak,
S.~Puglia\thanksref{l_CTUNI}\textsuperscript{,}\thanksref{l_CTINFN}\nolinebreak,
M.~Queiroga Bazetto\thanksref{l_Liverpool}\nolinebreak,
F.~Raffaelli\thanksref{l_PIINFN}\nolinebreak,
F.~Ragusa\thanksref{l_MIUni}\textsuperscript{,}\thanksref{l_MIINFN}\nolinebreak,
Y.~Ramachers\thanksref{l_Warwick}\nolinebreak,
A.~Ramirez\thanksref{l_Houston}\nolinebreak,
S.~Ravinthiran\thanksref{l_Liverpool}\nolinebreak,
M.~Razeti\thanksref{l_CAINFN}\nolinebreak,
A.~L.~Renshaw\thanksref{l_Houston}\nolinebreak,
A.~Repond\thanksref{l_UCRiverside}\nolinebreak,
M.~Rescigno\thanksref{l_RMUnoINFN}\nolinebreak,
S.~Resconi\thanksref{l_MIINFN}  \nolinebreak,
F.~Retiere\thanksref{l_TRIUMF}\nolinebreak,
L.~P.~Rignanese\thanksref{l_BOINFN}\nolinebreak,
A.~Ritchie-Yates\thanksref{l_Manchester}\nolinebreak,
A.~Rivetti\thanksref{l_TOINFN}\nolinebreak,
A.~Roberts\thanksref{l_Liverpool}\nolinebreak,
C.~Roberts\thanksref{l_Manchester}\nolinebreak,
G.~Rogers\thanksref{l_Birmingham}\nolinebreak,
L.~Romero\thanksref{l_CIEMAT}\nolinebreak,
M.~Rossi\thanksref{l_GEINFN}\nolinebreak,
A.~Rubbia\thanksref{l_ETHZ}\nolinebreak,
D.~Rudik\thanksref{l_NAUniPHY}\textsuperscript{,}\thanksref{l_NAINFN}\textsuperscript{,}\thanksref{l_MEPhI}\nolinebreak,
J.~Runge\thanksref{l_UMass}\nolinebreak,
M.~A.~Sabia\thanksref{l_RMUnoUni}\textsuperscript{,}\thanksref{l_RMUnoINFN}\textsuperscript{,}\thanksref{l_AstroCeNT}\nolinebreak,
P.~Salomone\thanksref{l_RMUnoUni}\textsuperscript{,}\thanksref{l_RMUnoINFN}\textsuperscript{,}\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_AstroCeNT}\nolinebreak,
O.~Samoylov\thanksref{l_JINR}\nolinebreak,
S.~Sanfilippo\thanksref{l_CTLNS}\nolinebreak,
D.~Santone\thanksref{l_Oxford}\nolinebreak,
R.~Santorelli\thanksref{l_CIEMAT}\nolinebreak,
E.~M.~Santos\thanksref{l_USP}\nolinebreak,
I.~Sargeant\thanksref{l_STFCppd}\nolinebreak,
C.~Savarese\thanksref{l_Washington}\nolinebreak,
E.~Scapparone\thanksref{l_BOINFN}\nolinebreak,
F.~G.~Schuckman\thanksref{l_Queens}\nolinebreak,
G.~Scioli\thanksref{l_BOUniPHY}\textsuperscript{,}\thanksref{l_BOINFN}\nolinebreak,
D.~A.~Semenov\thanksref{l_Petersburg}\nolinebreak,
V.~Shalamova\thanksref{l_UCRiverside}\nolinebreak,
S.~Sharma Poudel\thanksref{l_Houston}\nolinebreak,
A.~Sheshukov\thanksref{l_JINR}\nolinebreak,
M.~Simeone\thanksref{l_NAUniCHE}\textsuperscript{,}\thanksref{l_NAINFN}\nolinebreak,
P.~Skensved\thanksref{l_Queens}\nolinebreak,
M.~D.~Skorokhvatov\thanksref{l_Kurchatov}\textsuperscript{,}\thanksref{l_MEPhI}\nolinebreak,
O.~Smirnov\thanksref{l_JINR}\nolinebreak,
T.~Smirnova\thanksref{l_UCRiverside}\nolinebreak,
B.~Smith\thanksref{l_TRIUMF}\nolinebreak,
F.~Spadoni\thanksref{l_PNNL}\nolinebreak,
M.~Spangenberg\thanksref{l_Warwick}\nolinebreak,
A.~Steri\thanksref{l_CAINFN}\textsuperscript{,}\thanksref{l_CAUniCHE}\nolinebreak,
V.~Stornelli\thanksref{l_AQLNGS}\textsuperscript{,}\thanksref{l_UnivAQ}\nolinebreak,
S.~Stracka\thanksref{l_PIINFN}\nolinebreak,
% S.~Sulis\thanksref{\CAINFN\thanksref{\CAUniEEE}
A.~Sung\thanksref{l_Princeton}\nolinebreak,
C.~Sunny\thanksref{l_AstroCeNT}\nolinebreak,
Y.~Suvorov\thanksref{l_NAUniPHY}\textsuperscript{,}\thanksref{l_NAINFN}\textsuperscript{,}\thanksref{l_Kurchatov}\nolinebreak,
A.~M.~Szelc\thanksref{l_UniversityofEdinburgh}\nolinebreak,
O.~Taborda \thanksref{l_AQGSSI}\nolinebreak,\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
R.~Tartaglia\thanksref{l_AQLNGS}\nolinebreak,
A.~Taylor\thanksref{l_Liverpool}\nolinebreak,
J.~Taylor\thanksref{l_Liverpool}\nolinebreak,
G.~Testera\thanksref{l_GEINFN}\nolinebreak,
K.~Thieme\thanksref{l_Hawaii}\nolinebreak,
A.~Thompson\thanksref{l_RHUL}\nolinebreak,
S.~Torres-Lara\thanksref{l_Houston}\nolinebreak,
A.~Tricomi\thanksref{l_CTUNI}\nolinebreak,\textsuperscript{,}\thanksref{l_CTINFN}\nolinebreak,
E.~V.~Unzhakov\thanksref{l_Petersburg}\nolinebreak,
M.~Van Uffelen\thanksref{l_Oxford}\nolinebreak, %END GRACE PERIOD 30/09/2025
T.~Viant\thanksref{l_ETHZ}\nolinebreak,
S.~Viel\thanksref{l_Carleton}\nolinebreak,
A.~Vishneva\thanksref{l_JINR}\nolinebreak,
R.~B.~Vogelaar\thanksref{l_VTech}\nolinebreak,
J.~Vossebeld\thanksref{l_Liverpool}\nolinebreak,
B.~Vyas\thanksref{l_Carleton}\nolinebreak,
M.~Wada\thanksref{l_AstroCeNT}\nolinebreak,
M.~Walczak\thanksref{l_AQGSSI}\nolinebreak,\textsuperscript{,}\thanksref{l_AQLNGS}\nolinebreak,
Y.~Wang\thanksref{l_IHEP}\textsuperscript{,}\thanksref{l_UCAS}\nolinebreak,
S.~Westerdale\thanksref{l_UCRiverside}\nolinebreak,
L.~Williams\thanksref{l_FortLewis}\nolinebreak,
M.~M.~Wojcik\thanksref{l_Krakow}\nolinebreak,
M.~Wojcik\thanksref{l_Lodz}\nolinebreak,
% Y.~Xie\thanksref{\IHEP\thanksref{\UCAS} % end 30/04/2025
C.~Yang\thanksref{l_IHEP}\textsuperscript{,}\thanksref{l_UCAS}\nolinebreak,
J.~Yin\thanksref{l_IHEP}\textsuperscript{,}\thanksref{l_UCAS}\nolinebreak,
A.~Zabihi\thanksref{l_AstroCeNT}\nolinebreak,
P.~Zakhary\thanksref{l_CTUNI}\textsuperscript{,}\thanksref{l_CTINFN}%\thanksref{l_AstroCeNT}\nolinebreak,
A.~Zani\thanksref{l_MIINFN}\nolinebreak,
Y.~Zhang\thanksref{l_IHEP}\nolinebreak,
T.~Zhu\thanksref{l_UCDavis}\nolinebreak, %end of grace period Nov. 30, 2025
A.~Zichichi\thanksref{l_BOUniPHY}\textsuperscript{,}\thanksref{l_BOINFN}\nolinebreak,
G.~Zuzel\thanksref{l_Krakow}\nolinebreak,
M.~P.~Zykova\thanksref{l_MendeleevUniverisity}\nolinebreak

\begin{enumerate}
\item{\TNFBK\label{l_TNFBK}}
\item{\Carleton\label{l_Carleton}}
\item{\label{l_AQGSSI}\AQGSSI}
\item{\label{l_AQLNGS}\AQLNGS}
\item{\AstroCeNT\label{l_AstroCeNT}}
\item{\CTINFN\label{l_CTINFN}}
\item{\CTUNI\label{l_CTUNI}}
\item{\USP\label{l_USP}}
\item{\PNNL\label{l_PNNL}}
\item{\Augustana\label{l_Augustana}}
\item{\TRIUMF\label{l_TRIUMF}}
\item{\Columbia\label{l_Columbia}}
\item{\CAINFN\label{l_CAINFN}}
\item{\CAUniPHY\label{l_CAUniPHY}}
\item{\Alberta\label{l_Alberta}}
\item{\MendeleevUniverisity\label{l_MendeleevUniverisity}}
\item{\LNLINFN\label{l_LNLINFN}}
\item{\SNL\label{l_SNL}}
\item{\RHUL\label{l_RHUL}}
\item{\CIEMAT\label{l_CIEMAT}}
\item{\CPPM\label{l_CPPM}}
\item{\PIINFN\label{l_PIINFN}}
\item{\PIUniPHY\label{l_PIUniPHY}}
\item{\Oxford\label{l_Oxford}}
\item{\TOINFN\label{l_TOINFN} }
\item{\TOPoli\label{l_TOPoli}}
\item{\RMUnoINFN\label{l_RMUnoINFN}}
\item{\GEUni\label{l_GEUni}}
\item{\GEINFN\label{l_GEINFN}}
\item{\MIPoliICA\label{l_MIPoliICA}}
\item{\MIINFN\label{l_MIINFN}}
\item{\WUT\label{l_WUT} }
\item{\RMTreINFN\label{l_RMTreINFN} }
\item{\NAINFN\label{l_NAINFN} }
\item{\VTech\label{l_VTech} }
\item{\CAUniEEE\label{l_CAUniEEE} }
\item{\Zaragoza\label{l_Zaragoza} }
\item{\MSU\label{l_MSU} }
\item{\BOINFN\label{l_BOINFN} }
\item{\BOUniPHY\label{l_BOUniPHY} }
\item{\Laurentian\label{l_Laurentian} }
\item{\SNOLAB\label{l_SNOLAB} }
\item{\AQUni\label{l_UnivAQ} }
\item{\Krakow\label{l_Krakow} }
\item{\NAUniDIST\label{l_NAUniDIST} }
\item{\MIUni\label{l_MIUni} }
\item{\RMUnoUni\label{l_RMUnoUni} }
\item{\MIPoliCHE\label{l_MIPoliCHE} }
\item{\Petersburg\label{l_Petersburg} }
\item{\NAUniPHY\label{l_NAUniPHY} }
\item{\Queens\label{l_Queens} }
\item{\Princeton\label{l_Princeton} }
\item{\Kurchatov\label{l_Kurchatov} }
\item{\Belgorod\label{l_Belgorod} }
\item{\UCDavis\label{l_UCDavis} }
\item{\Lancaster\label{l_Lancaster} }
\item{\APC\label{l_APC} }
\item{\Liverpool\label{l_Liverpool} }
\item{\BINP\label{l_BINP} }
\item{\BOCentroFermi\label{l_BOCentroFermi} }
\item{\Manchester\label{l_Manchester} }
\item{\ETHZ\label{l_ETHZ} }
\item{\WilliamsCollege\label{l_WilliamsCollege} }
\item{\Hawaii\label{l_Hawaii} }
\item{\Chicago\label{l_Chicago} }
\item{\CTLNS\label{l_CTLNS} }
\item{\IHEP\label{l_IHEP} }
\item{\UniversityofEdinburgh\label{l_UniversityofEdinburgh} }
\item{\Houston\label{l_Houston} }
\item{\NAUniPHARM\label{l_NAUniPHARM} }
\item{\UCRiverside\label{l_UCRiverside} }
\item{\JINR\label{l_JINR} }
\item{\MEPhI\label{l_MEPhI} }
\item{\Birmingham\label{l_Birmingham} }
\item{\UniHAM\label{l_UniHAM} }
%\item{\LFoundry\label{l_LFoundry} }
\item{\Temple\label{l_Temple} }
\item{\Warwick\label{l_Warwick} }
\item{\INFN\label{l_INFN} }
\item{\UMass\label{l_UMass} }
\item{\NAUniCHE\label{l_NAUniCHE} }
\item{\CAUniCHE\label{l_CAUniCHE} }
\item{\UCAS\label{l_UCAS} }
\item{\UCLA\label{l_UCLA} }
\item{\FortLewis\label{l_FortLewis} }
\item{\Lodz\label{l_Lodz}}
\item{\STFCInterconnect\label{l_STFCInterconnect}}
\item{\ENUniCEE\label{l_ENUniCEE}}
%\item{\Seattle\label{l_Seattle}}
\item{\STFCppd\label{l_STFCppd}}
\item{\RMTreUni\label{l_RMTreUni}}
\item{\Washington\label{l_Washington}}
\end{enumerate}

}

==> inst-july2025.tex <==
\newcommand{\Alberta}{Department of Physics, University of Alberta, Edmonton, AB T6G 2R3, Canada}
\newcommand{\APC}{APC, Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, Paris F-75013, France}
\newcommand{\AQLNGS}{INFN Laboratori Nazionali del Gran Sasso, Assergi (AQ) 67100, Italy}
\newcommand{\AQGSSI}{Gran Sasso Science Institute, L'Aquila 67100, Italy}
\newcommand{\AQUni}{
Department of Industrial and Information Engineering and Economics, Università degli Studi dell'Aquila, L'Aquila 67100, Italy}
\newcommand{\AstroCeNT}{AstroCeNT, Nicolaus Copernicus Astronomical Center of the Polish Academy of Sciences, 00-614 Warsaw, Poland}
\newcommand{\Augustana}{Physics Department, Augustana University, Sioux Falls, SD 57197, USA}
\newcommand{\Belgorod}{Radiation Physics Laboratory, Belgorod National Research University, Belgorod 308007, Russia}
\newcommand{\BHSU}{School of Natural Sciences, Black Hills State University, Spearfish, SD 57799, USA}
\newcommand{\BINP}{Budker Institute of Nuclear Physics, Novosibirsk 630090, Russia}
\newcommand{\Birmingham}{School of Physics and Astronomy, University of Birmingham, Edgbaston, B15 2TT, Birmingham, UK}
\newcommand{\BNLaddress}{Brookhaven National Laboratory, Upton, NY 11973, USA}
\newcommand{\BOINFN}{INFN Bologna, Bologna 40126, Italy}
\newcommand{\BOUniPHY}{Department of Physics and Astronomy, Universit\`a degli Studi di Bologna, Bologna 40126, Italy}
\newcommand{\CAUniCHE}{Department of Mechanical, Chemical, and Materials Engineering, Universit\`a degli Studi, Cagliari 09042, Italy}
\newcommand{\CAUniEEE}{Department of Electrical and Electronic Engineering, Universit\`a degli Studi di Cagliari, Cagliari 09123, Italy}
\newcommand{\CAUniPHY}{Physics Department, Universit\`a degli Studi di Cagliari, Cagliari 09042, Italy}
\newcommand{\CAINFN}{INFN Cagliari, Cagliari 09042, Italy}
\newcommand{\Carleton}{Department of Physics, Carleton University, Ottawa, ON K1S 5B6, Canada}
\newcommand{\Campinas}{Physics Institute, Universidade Estadual de Campinas, Campinas 13083, Brazil}
\newcommand{\Columbia}{Physics Department, Columbia University, New York, NY 10027, USA}
\newcommand{\Chicago}{Department of Physics and Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\newcommand{\BOCentroFermi}{Museo Storico della Fisica e Centro Studi e Ricerche Enrico Fermi, Roma 00184, Italy}
\newcommand{\CERNaddress}{CERN, European Organization for Nuclear Research 1211 Geneve 23, Switzerland, CERN}
\newcommand{\CIEMAT}{CIEMAT, Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, Madrid 28040, Spain}
\newcommand{\Cluj}{National Institute for R\&D of Isotopic and Molecular Technologies, Cluj-Napoca, 400293, Romania}
\newcommand{\CPPM}{Centre de Physique des Particules de Marseille, Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}
\newcommand{\CTINFN}{INFN Catania, Catania 95121, Italy}
\newcommand{\CTUNI}{Universit\`a of Catania, Catania 95124, Italy}
\newcommand{\CTLNS}{INFN Laboratori Nazionali del Sud, Catania 95123, Italy}
\newcommand{\ENSMP}{\'Ecole nationale sup\'erieure des mines de Paris, Paris 75272, France}
\newcommand{\ENUniCEE}{Engineering and Architecture Department, Universit\`a di Enna Kore, Enna 94100, Italy}
\newcommand{\ETHZ}{Institute for Particle Physics and Astrophysics, ETH Zurich, Zurich 8093, Switzerland}
\newcommand{\FNAL}{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\newcommand{\FortLewis}{Department of Physics and Engineering, Fort Lewis College, Durango, CO 81301, USA}
\newcommand{\GEUni}{Physics Department, Universit\`a degli Studi di Genova, Genova 16146, Italy}
\newcommand{\GEINFN}{INFN Genova, Genova 16146, Italy}
\newcommand{\Hawaii}{Department of Physics and Astronomy, University of Hawai'i, Honolulu, HI 96822, USA}
\newcommand{\Houston}{Department of Physics, University of Houston, Houston, TX 77204, USA}
\newcommand{\IHEP}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\INFN}{Istituto Nazionale di Fisica Nucleare, Roma 00186, Italia}
\newcommand{\IPNO}{Institut de Physique Nucl\`eaire d'Orsay, 91406, Orsay, France}
\newcommand{\INSTM}{Interuniversity Consortium for Science and Technology of Materials, Firenze 50121, Italy}
\newcommand{\IPHC}{IPHC, Universit\'e de Strasbourg, CNRS/IN2P3, Strasbourg 67037, France}
\newcommand{\JINR}{Joint Institute for Nuclear Research, Dubna 141980, Russia}
\newcommand{\Krakow}{M.~Smoluchowski Institute of Physics, Jagiellonian University, 30-348 Krakow, Poland}
\newcommand{\Kurchatov}{National Research Centre Kurchatov Institute, Moscow 123182, Russia}
\newcommand{\Laurentian}{Department of Physics and Astronomy, Laurentian University, Sudbury, ON P3E 2C6, Canada}
\newcommand{\Lancaster}{Physics Department, Lancaster University, Lancaster LA1 4YB, UK}
\newcommand{\Liverpool}{Department of Physics, University of Liverpool, The Oliver Lodge Laboratory, Liverpool L69 7ZE, UK}
\newcommand{\LNFINFN}{INFN Laboratori Nazionali di Frascati, Frascati 00044, Italy}
\newcommand{\LNLINFN}{INFN Laboratori Nazionali di Legnaro, Legnaro (Padova) 35020, Italy}
\newcommand{\Lodz}{Institute of Applied Radiation Chemistry, Lodz University of Technology, 93-590 Lodz, Poland}
\newcommand{\LPNHE}{LPNHE, CNRS/IN2P3, Sorbonne Universit\'e, Universit\'e Paris Diderot, Paris 75252, France}
\newcommand{\Mainz}{Institut f\"ur Kernphysik, Johannes Gutenberg-Universit\"at Mainz, D-55128 Mainz, Germany}
\newcommand{\Manchester}{Department of Physics and Astronomy, The University of Manchester, Manchester M13 9PL, UK}
\newcommand{\MEPhI}{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\newcommand{\MendeleevUniverisity}{Mendeleev University of Chemical Technology, Moscow 125047, Russia}
\newcommand{\MIBIINFN}{INFN Milano Bicocca, Milano 20126, Italy}
\newcommand{\MIINFN}{INFN Milano, Milano 20133, Italy}
\newcommand{\MIPoliICA}{Civil and Environmental Engineering Department, Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIPoliCHE}{Chemistry, Materials and Chemical Engineering Department ``G.~Natta", Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIPoliEIB}{Electronics, Information, and Bioengineering Department, Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIPoliENE}{Energy Department, Politecnico di Milano, Milano 20133, Italy}
\newcommand{\MIUni}{Physics Department, Universit\`a degli Studi di Milano, Milano 20133, Italy}
\newcommand{\MSU}{Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Moscow 119234, Russia}
\newcommand{\NAINFN}{INFN Napoli, Napoli 80126, Italy}
\newcommand{\NAUniPHY}{Physics Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80126, Italy}
\newcommand{\NAUniCHE}{Chemical, Materials, and Industrial Production Engineering Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80126, Italy}
\newcommand{\NAUniDIST}{Department of Structures for Engineering and Architecture, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80126, Italy}
\newcommand{\NAUniPHARM}{Pharmacy Department, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80131, Italy}
\newcommand{\NAUniStruct}{Department of Strutture per l'Ingegneria e l'Architettura, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80131, Italy}
\newcommand{\NAUniEEIT}{Department of Electrical Engineering and Information Technology, Universit\`a degli Studi ``Federico II'' di Napoli, Napoli 80125, Italy}
\newcommand{\NSU}{Novosibirsk State University, Novosibirsk 630090, Russia}
\newcommand{\OACINAF}{INAF Osservatorio Astronomico di Capodimonte, 80131 Napoli, Italy}
\newcommand{\Oxford}{University of Oxford, Oxford OX1 2JD, United Kingdom}
\newcommand{\Petersburg}{Saint Petersburg Nuclear Physics Institute, Gatchina 188350, Russia}
\newcommand{\PGUniCBB}{Chemistry, Biology and Biotechnology Department, Universit\`a degli Studi di Perugia, Perugia 06123, Italy}
\newcommand{\PGINFN}{INFN Perugia, Perugia 06123, Italy}
\newcommand{\PIINFN}{INFN Pisa, Pisa 56127, Italy}
\newcommand{\PIUniPHY}{Physics Department, Universit\`a degli Studi di Pisa, Pisa 56127, Italy}
\newcommand{\PNNL}{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\newcommand{\Princeton}{Physics Department, Princeton University, Princeton, NJ 08544, USA}
\newcommand{\Queens}{Department of Physics, Engineering Physics and Astronomy, Queen's University, Kingston, ON K7L 3N6, Canada}
\newcommand{\RHUL}{Department of Physics, Royal Holloway University of London, Egham TW20 0EX, UK}
\newcommand{\RMTreINFN}{INFN Roma Tre, Roma 00146, Italy}
\newcommand{\RMTreUni}{Department of Mathematics and Physics – Roma Tre University, Roma 00146, Italy}
\newcommand{\RMUnoINFN}{INFN Sezione di Roma, Roma 00185, Italy}
\newcommand{\RMUnoUni}{Physics Department, Sapienza Universit\`a di Roma, Roma 00185, Italy}
\newcommand{\SAINFN}{INFN Salerno, Salerno 84084, Italy}
\newcommand{\SNL}{Savannah River National Laboratory, Jackson, SC 29831, United States}
\newcommand{\SAUni}{Physics Department, Universit\`a degli Studi di Salerno, Salerno 84084, Italy}
\newcommand{\SNOLAB}{SNOLAB, Lively, ON P3Y 1N2, Canada}
\newcommand{\SSUniCHP}{Chemistry and Pharmacy Department, Universit\`a degli Studi di Sassari, Sassari 07100, Italy}
\newcommand{\STFCInterconnect}{Science \& Technology Facilities Council (STFC), Rutherford Appleton Laboratory, Technology, Harwell Oxford, Didcot OX11 0QX, UK}
\newcommand{\STFCppd}{Science \& Technology Facilities Council (STFC), Rutherford Appleton Laboratory, Particle Physics Department, Harwell Oxford, Didcot OX11 0QX, UK}
\newcommand{\Sussex}{Physics and Astronomy Department, University of Sussex, Brighton BN1 9QH, UK}
\newcommand{\Temple}{Physics Department, Temple University, Philadelphia, PA 19122, USA}
\newcommand{\TNFBK}{Fondazione Bruno Kessler, Povo 38123, Italy}
\newcommand{\TNTIFPA}{Trento Institute for Fundamental Physics and Applications, Povo 38123, Italy}
\newcommand{\TNUni}{Physics Department, Universit\`a degli Studi di Trento, Povo 38123, Italy}
\newcommand{\TOINFN}{INFN Torino, Torino 10125, Italy}
\newcommand{\TOPoli}{Department of Electronics and Telecommunications, Politecnico di Torino, Torino 10129, Italy}
\newcommand{\TOUni}{Physics Department, Universit\`a degli Studi di Torino, Torino 10125, Italy}
\newcommand{\TRIUMF}{TRIUMF, 4004 Wesbrook Mall, Vancouver, BC V6T 2A3, Canada}
\newcommand{\TUM}{Physik Department, Technische Universit\"at M\"unchen, Munich 80333, Germany}
\newcommand{\UB}{Universiatat de Barcelona, Barcelona E-08028, Catalonia, Spain} 
\newcommand{\UCDavis}{Department of Physics, University of California, Davis, CA 95616, USA}
\newcommand{\UCRiverside}{Department of Physics and Astronomy, University of California, Riverside, CA 92507, USA}
\newcommand{\UCSanDiego}{Department of Physics, University of California, San Diego, CA 92093, USA}
\newcommand{\UCLA}{Physics and Astronomy Department, University of California, Los Angeles, CA 90095, USA}
\newcommand{\UCAS}{University of Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\UMass}{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\newcommand{\UNAM}{Instituto de F\'isica, Universidad Nacional Aut\'onoma de M\'exico, M\'exico 01000, Mexico}
\newcommand{\UnivAQ}{Universit\`a degli Studi dell’Aquila, L’Aquila 67100, Italy}
\newcommand{\UniversityofEdinburgh}{School of Physics and Astronomy, University of Edinburgh, Edinburgh EH9 3FD, UK}
\newcommand{\UOC}{Department of Chemistry, University of Crete, P.O. Box 2208, 71003 Heraklion, Crete, Greece}
\newcommand{\USP}{Instituto de F\'isica, Universidade de S\~ao Paulo, S\~ao Paulo 05508-090, Brazil}
\newcommand{\VTech}{Virginia Tech, Blacksburg, VA 24061, USA}
\newcommand{\Washington}{Center for Experimental Nuclear Physics and Astrophysics, and Department of Physics, University of Washington, Seattle, WA 98195, USA}
\newcommand{\Warwick}{University of Warwick, Department of Physics, Coventry CV47AL, UK}
\newcommand{\WUT}{Institute of Radioelectronics and Multimedia Technology, Faculty of Electronics and Information Technology, Warsaw University of Technology, 00-661 Warsaw, Poland}
%\newcommand{\WUT}{Institute of Radioelectronics and Multimedia Technology, Faculty of Electronics and Information Technology, Warsaw University of Technology, Nowowiejska 15/19, 00-661 Warsaw, Poland}
%\newcommand{\WUT}{Warsaw University of Technology, 00-661 Warsaw, Poland}
\newcommand{\WilliamsCollege}{Williams College, Department of Physics and Astronomy, Williamstown, MA 01267 USA}
\newcommand{\Zaragoza}{Centro de Astropart\'iculas y F\'isica de Altas Energ\'ias, Universidad de Zaragoza, Zaragoza 50009, Spain}
\newcommand{\ZaragozaARAID}{Fundaci\'on ARAID, Universidad de Zaragoza, Zaragoza 50009, Spain}
\newcommand{\UniHAM}{Institute of Experimental Physics, University of Hamburg, Luruper Chaussee 149, 22761, Hamburg, Germany}
\newcommand{\SDakota}{School of Natural Sciences, Black Hills State University, Spearfish, South Dakota 57799, USA}
\newcommand{\Saclay}{Universit\´e Paris-Saclay, CEA, List, Laboratoire National Henri Becquerel (LNE-LNHB),
F-91120 Palaiseau, France}
\newcommand{\NASS}{Scuola Superiore Meridionale,  80138 Napoli, Italy}
